Tight Bounds on List-Decodable and List-Recoverable Zero-Rate Codes

In this work, we consider the list-decodability and list-recoverability of codes in the zero-rate regime. Briefly, a code $\mathcal{C} \subseteq [q]^n$ is $(p,\ell,L)$-list-recoverable if for all tuples of input lists $(Y_1,\dots,Y_n)$ with each $Y_i \subseteq [q]$ and $|Y_i|=\ell$ the number of codewords $c \in \mathcal{C}$ such that $c_i \notin Y_i$ for at most $pn$ choices of $i \in [n]$ is less than $L$; list-decoding is the special case of $\ell=1$. In recent work by Resch, Yuan and Zhang~(ICALP~2023) the zero-rate threshold for list-recovery was determined for all parameters: that is, the work explicitly computes $p_*:=p_*(q,\ell,L)$ with the property that for all $\epsilon>0$ (a) there exist infinite families positive-rate $(p_*-\epsilon,\ell,L)$-list-recoverable codes, and (b) any $(p_*+\epsilon,\ell,L)$-list-recoverable code has rate $0$. In fact, in the latter case the code has constant size, independent on $n$. However, the constant size in their work is quite large in $1/\epsilon$, at least $|\mathcal{C}|\geq (\frac{1}{\epsilon})^{O(q^L)}$. Our contribution in this work is to show that for all choices of $q,\ell$ and $L$ with $q \geq 3$, any $(p_*+\epsilon,\ell,L)$-list-recoverable code must have size $O_{q,\ell,L}(1/\epsilon)$, and furthermore this upper bound is complemented by a matching lower bound $\Omega_{q,\ell,L}(1/\epsilon)$. This greatly generalizes work by Alon, Bukh and Polyanskiy~(IEEE Trans.\ Inf.\ Theory~2018) which focused only on the case of binary alphabet (and thus necessarily only list-decoding). We remark that we can in fact recover the same result for $q=2$ and even $L$, as obtained by Alon, Bukh and Polyanskiy: we thus strictly generalize their work.

==> tmp.tex <==

\section{Lee codes}
A motivation of looking into codes w.r.t.\ the Lee metric ($d_{\mathrm{Lee}}(a,b) = \min\brace{|a - b|, q - |a - b|}$ for $a,b\in[q]$) is that this metric is an affine function which allows the trick \cite{abp-2018} of applying minimax theorem to the Chebyshev radius to go through. 
The first step is to determine the zero-rate threshold. 
I would expect the following heuristic to yield the truth. 
Sample $L$ codewords independently, each entry i.i.d.\ according to a distribution $P\in\Delta([q])$. 
(Here $P$ needs to be the optimal input distribution. A priori I don't know if it should be $\unif$, but we can optimize it in the end.)
Compute the average radius $np$ of these $L$ codewords. 
I expect that the resulting $p$ is the right zero-rate threshold. 

\begin{itemize}
    \item The choice for the ``centroid'' of the Lee metric seems to be essentially the median of the coordinate values, but we have to be careful about ``wrapping around.''

    \item Make the above argument regarding zero-rate threshold rigorous. 
    To do so, we need to carry out the first moment (i.e., double-counting) method. 

    \item Capacity upper bound using Elias--Bassalygo + covering. 
    My impression is that it is tricky to compute the normalized log-volume of a Lee ball. 
    (Note that the volume is independent of the center.)
    I saw some references \cite{ByrneWeger_Lee,Decode_Lee} that do so by considering certain generating functions. 

    \item Capacity lower bounds using expurgation. 

    \item Carry out the ABP argument. 
    I'm interested in seeing any setting in which one can bypass the Ramsey reduction and obtain $\poly(1/\eps)$-bounds for codes $\eps$-above the zero-rate threshold. 

    \item For list-size $1$, is there a chance to prove an LP bound?
    I think (check) the Lee metric does give rise to an association scheme. 
    First for linear codes, then from linear to general codes. 

    \begin{itemize}
        \item If one can pull off the above, then even more ambitiously, Polyanskiy \cite{polyanskiy-2016-list-dec} has an improvement on the EB upper bound for list-decoding in the low-rate regime. 
        This is relies on the (unique-decoding) LP bound (in fact perhaps something more involved than that -- bounds on distance distribution). 
    \end{itemize}

    \item Efficient/explicit constructions. I'm not so familiar but Nic/Chen might be. 
\end{itemize}

How much of the above has already been known in the literature?
(I assume not much in the constant list-size regime, but need to check anyways.)
Other motivations for Lee codes from crypto, flash memory?

\section{List-recoverable codes}

